Lower Bound Techniques in the Comparison-Query Model and Inversion Minimization on Trees

Given a rooted tree and a ranking of its leaves, what is the minimum number of inversions of the leaves that can be attained by ordering the tree? This variation of the problem of counting inversions in arrays originated in mathematical psychology, with the evaluation of the Mann--Whitney statistic for detecting differences between distributions as a special case. We study the complexity of the problem in the comparison-query model, used for problems like sorting and selection. For many types of trees with $n$ leaves, we establish lower bounds close to the strongest known in the model, namely the lower bound of $\log_2(n!)$ for sorting $n$ items. We show: (a) $\log_2((\alpha(1-\alpha)n)!) - O(\log n)$ queries are needed whenever the tree has a subtree that contains a fraction $\alpha$ of the leaves. This implies a lower bound of $\log_2((\frac{k}{(k+1)^2}n)!) - O(\log n)$ for trees of degree $k$. (b) $\log_2(n!) - O(\log n)$ queries are needed in case the tree is binary. (c) $\log_2(n!) - O(k \log k)$ queries are needed for certain classes of trees of degree $k$, including perfect trees with even $k$. The lower bounds are obtained by developing two novel techniques for a generic problem $\Pi$ in the comparison-query model and applying them to inversion minimization on trees. Both techniques can be described in terms of the Cayley graph of the symmetric group with adjacent-rank transpositions as the generating set. Consider the subgraph consisting of the edges between vertices with the same value under $\Pi$. We show that the size of any decision tree for $\Pi$ must be at least: (i) the number of connected components of this subgraph, and (ii) the factorial of the average degree of the complementary subgraph, divided by $n$. Lower bounds on query complexity then follow by taking the base-2 logarithm.

==> binary.tex <==
\section{Binary Trees}
\label{sec:binary}

In this section we establish our results on the query complexity of minimizing inversions on binary trees. We fix a binary tree $T$ with $n$ leaves, and consider the problem $\Pi_T(\ranking) = \MInv(T,\ranking)$ in the comparison-based model with the leaves of $T$ as the items, i.e., $X = L(T)$. We first develop a criterion for when a particular ranking $\ranking$ is sensitive to a particular adjacent-rank transposition $\transposition$, of equivalently, for when an edge in the permutahedron is monochromatic with respect to $\Pi_T$ and thus belongs to the permutahedron graph $G(\Pi_T)$, or else is bichromatic and therefore belongs to the complementary permutahedron graph $\overline{G}(\Pi_T)$. We then employ this criterion in an application of the Connectivity Lemma (leading to part (b) of Theorem~\ref{thm:main:binary}) and in an application of the Sensitivity Lemma (leading to part (a) of Theorem~\ref{thm:main:binary}).

\paragraph{Decomposition of the objective function} 
We start with an analysis for an arbitrary tree $T$. Recall that the objective $\MInv(T,\ranking)$ can be decomposed into contributions of individual nodes. The contribution of a node $v$ is those inversions that reside in the subtree $T_v$ and go through the root $v$ of $T_v$. We refer to them as the root inversions in $T_v$. 
\begin{definition}[root inversions, $\RInv$, $\MRInv$]
Given a tree $T$, a ranking $\ranking$ of the leaves of $T$, and an ordering $\ordering$ of $T$, a root inversion of $\ordering$ with respect to $\ranking$ is an inversion of $\ordering$ with respect to $\ranking$ for which the affected leaves have the root of $T$ as their lowest common ancestor. The number of root inversions of $\ordering$ with respect to $\ranking$ in $T$ is denoted by $\RInv(T,\ranking,\ordering)$. The minimum number of root inversion in $T$ with respect to $\ranking$ is denoted 
\begin{equation}\label{eq:MRInv}
\MRInv(T,\ranking) \doteq \min_\ordering \RInv(T,\ranking,\ordering),
\end{equation}
where $\ordering$ ranges over all possible orderings of $T$.
\end{definition}
The only aspect of the ordering $\ordering$ of $T_v$ that affects $\RInv(T_v,\ranking,\ordering)$ is the relative order of the children of $v$. For a node $v$ with $k$ children $u_1,\dots,u_k$, by abusing notation and using $\ordering$ to also denote the ranking of the children induced by the ordering of the tree, we have
\begin{equation}\label{eq:cost}
\RInv(T,\ranking,\ordering) \doteq \sum_{1 \le i < j \le k} \XInv_\ranking(L_{\ordering(i)},L_{\ordering(j)}),
\end{equation}
where $L_i$ is a short-hand for the leaf set $L(T_{u_i})$. The contributions of the nodes can be optimized independently:
\begin{equation}\label{eq:MInv:decomposition}
\MInv(T,\ranking) = \sum_v \MRInv(T_v,\ranking),
\end{equation}
where $v$ ranges over all nodes of $T$ with degree $\deg_T(v)>1$. 

In the case of binary trees, we only need to consider nodes $v$ of degree 2, for which there are only two possible rankings of its children, $u_1$ and $u_2$, with leaf sets $L_1 = L(T_{u_1})$ and $L_2 = L(T_{u_2})$:
\begin{equation}\label{eq:contribution:binary:retake}
\MRInv(T_v,\ranking) = \min(\XInv_\ranking(L_1,L_2),\XInv_\ranking(L_2,L_1)).
\end{equation}
This makes an explicit analysis of sensitivity feasible, as we will see next. 

\subsection{Sensitivity criterion}
\label{sec:binary:criterion}

For a given ranking $\ranking$ of $T$ and a given adjacent-rank transposition $\transposition$, we would like to figure out the effect of $\transposition$ on the objective $\MInv(T,\cdot)$, in particular when $\MInv(T,\transposition \circ \ranking) = \MInv(T,\ranking)$. 
Let $\ell_\lo$ and $\ell_\hi$ denote the two leaves that are affected by the transposition $\transposition$ on ranking $\ranking$, where 
the subscript "$\lo$" indicates the lower of the two leaves with respect to $\ranking$, and "$\hi$" the higher of the two. Let 
$v$ be the lowest common ancestor $\LCA(\ell_\lo,\ell_\hi)$.
We use the same subscripts "$\lo$" and "$\hi$"for the two children of $v$, where $u_\lo$ denotes the child whose subtree contains $\ell_\lo$, and $u_\hi$ its sibling, and similarly for the leave sets $L_\lo$ and $L_\hi$. See Figure~\ref{fig:sensitivity:binary} for the subsequent analysis. 

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \node (top) at (0,0)[circle,draw,fill=black,inner sep=2pt,label={above:$v$}]{};
        \node (ulo) at (-1.5,-1)[circle,draw,fill=black,inner sep=2pt,label={left:$u_{\lo}$}]{};
        \node (uhi) at (1.5,-1)[circle,draw,fill=black,inner sep=2pt,label={right:$u_{\hi}$}]{};
        \node (llo) at (-2,-4)[circle,draw,fill=black,inner sep=2pt,label={left:$\ell_{\lo}$}]{};
        \node (lhi) at (2,-4)[circle,draw,fill=black,inner sep=2pt,label={right:$\ell_{\hi}$}]{};
        
        \draw (ulo) -- (top) -- (uhi);
        \draw[decorate, decoration=snake] (ulo) -- (llo);
        \draw[decorate, decoration=snake] (uhi) -- (lhi);
        
        \draw (llo) ellipse (1.4 and 0.7);
        \draw (lhi) ellipse (1.4 and 0.7);
        
        % TODO
        \draw [dashed] (ulo)--(-3.4,-4);
    \end{tikzpicture}
    \caption{Sensitivity analysis for binary trees}
    \label{fig:sensitivity:binary}
\end{figure}

For any leaf $\ell$ other than $\ell_\lo$ and $\ell_\hi$, the relative order of $\ell$ under $\ranking$ is the same with respect to $\ell_\lo$ as it is with respect to $\ell_\hi$. This means that the adjacent-rank transposition $\transposition$ does not affect whether a pair of leaves $\{\ell_1,\ell_2\}$ constitutes an inversion unless $\{\ell_1,\ell_2\} = \{\ell_\lo,\ell_hi\}$. As a result, the only term on the right-hand side of \eqref{eq:MInv:decomposition} that can be affected by the transposition $\transposition$ is the one corresponding to the node $v$, and it can change by at most one unit. The situation before and after the application of $\transposition$ is as follows, where $x \doteq \XInv_\ranking(L_\lo,L_\hi)$ and $y \doteq \XInv_\ranking(L_\hi,L_\lo)$. 

\begin{equation*}
    \begin{array}{c|cc|c}
      \text{ranking} & \RInv(T_v,\cdot, \ell_\lo < \ell_\hi) &  \RInv(T_v,\cdot, \ell_\hi < \ell_\lo) & \MRInv(T_v,\cdot) \\
      \hline
      \ranking & x & y & \min(x,y) \\
      \ranking \circ \transposition & y-1 & x+1 & \min(y-1,x+1)
    \end{array}
\end{equation*}

The objective function remains the same iff $\min(x,y) = \min(y-1,x+1)$, which happens iff $x-y+1=0$, or equivalently iff
\begin{equation}\label{eq:criterion:derivation}
\DInv_\ranking(L_\lo,L_\hi) - \DInv_\ranking(\{\ell_\lo\},\{\ell_\hi\}) = 0,
\end{equation}
where we introduce the following short-hand: 
\begin{definition}[cross inversion difference, $\DInv$]
For a ranking $\ranking$ of a set $X$, and two subsets $A, B \subseteq X$,
\[ \DInv_\ranking(A,B) \doteq \XInv_\ranking(A,B) - \XInv_\ranking(B,A). \]
\end{definition}
We can split $L_\lo$ as $L_\lo = \{\ell_\lo\} \sqcup A = A_< \sqcup \{\ell_\lo\} \sqcup A_>$, where $A_<$ contains all leaves in $L_\lo$ that $\ranking$ ranks before $\ell_\lo$, and $A_>$ contains all the leaves in $L_\lo$ that $\ranking$ ranks after $\ell_\lo$. We similarly split $L_\hi$, as indicated in Figure~\ref{fig:sensitivity:binary}. We have that
\[ \DInv_\ranking(L_\lo,L_\hi) = \DInv_\ranking(\{\ell_\lo\},\{\ell_\hi\}) + \DInv_\ranking(\{\ell_\lo\},B) + \DInv_\ranking(A,\{\ell_\hi\}) + \DInv_\ranking(A,B).\]
Since the ranks of $\ell_\lo$ and $\ell_\hi$ under $\ranking$ are adjacent, we have that $\DInv_\ranking(\{\ell_\lo\},B) = |B_<| - |B_>|$ and $\DInv_\ranking(A,\{\ell_\hi\}) = |A_>| - |A_<|$. Plugging everything into \eqref{eq:criterion:derivation} we conclude:

\begin{proposition}
Let $T$ be a binary tree, $\ranking$ a ranking of the leaves of $T$, $\transposition$ an adjacent-rank transposition, $\ell_\lo$ and $\ell_\hi$ the two leaves affected by $\transposition$ under $\ranking$ such that $\ranking$ ranks $\ell_\lo$ before $\ell_\hi$. Referring to the notation in Figure~\ref{fig:sensitivity:binary}, we have that 
\begin{equation}\label{eq:criterion:binary}
\MInv(T,\ranking) = \MInv(T,\ranking \circ \transposition)
\Leftrightarrow \DInv_\ranking(A,B) = |A_<| - |A_>| + |B_>| - |B_<|.
\end{equation}
\end{proposition}

\subsection{Connectivity}
\label{sec:binary:connectivity}

\subsection{Average sensitivity}
\label{sec:binary:sensitivity}





==> connectivity.tex <==
\section{Connectivity}
\label{sec:connectivity}

In this section we establish the Connectivity Lemma and use it to present some of the known lower bounds in a unified framework. In fact, we prove the following somewhat stronger lemma.

\begin{lemma}\label{lemma:connectivity:strong}
Consider an execution trace of an algorithm for a problem $\Pi$ in the comparison-based model, and the set $R$ of all rankings that induce this execution trace. The set $R$ is connected in $G(\Pi)$.
\end{lemma}
The Connectivity Lemma follows from Lemma~\ref{lemma:connectivity:strong} because an execution traces dictates the output, which means that the set $R$ needs to be part of a connected component of $G(\Pi)$. 

\begin{proof}[Proof of Lemma~\ref{lemma:connectivity:strong}]
For any two rankings $\ranking_1, \ranking_2 \in R$, we construct a path from $\ranking_1$ to $\ranking_2$ in $G(\Pi)$ that stays entirely within $R$.

If $\ranking_1 = \ranking_2$, we do not need to make any move and use an empty path. 

Otherwise, there exists a rank $r<n$ such that $\ranking_1$ and $\ranking_2$ agree on ranks less than $r$ and disagree on rank $r$. We have the following situation, where the item $y_r$ with rank $r$ under $\ranking_2$, has rank $s>r$ under $\ranking_1$. 

 \begin{equation*}
    \begin{array}{r|ccccccccc}
      \text{rank} & 1 & \cdots &  r-1 &   r & \cdots & s-1 & s & \cdots &   n \\
      \hline
      \ranking_1^{-1} & x_1 & \cdots & x_{r-1} &   x_r  & \cdots & x_{s-1} & x_s = y_r & \cdots &     \\
       & {\scriptstyle =}  & {\scriptstyle =}  & {\scriptstyle =}  &  {\scriptstyle \ne}  &    &    &  &   &    \\
      \ranking_2^{-1} & y_1 & \cdots & y_{r-1} & y_r & \cdots &     &     & \cdots &    
    \end{array}
  \end{equation*}

Considering ranking $\ranking_1$, we have that $\ranking_1(x_{s-1}) = s-1 < s = \ranking_1(x_s)$. Considering ranking $\ranking_2$, since $x_{s-1}$ differs from $y_i=x_i$ for every $i \in [r-1]$ and also differs from $y_r$, we have that $\ranking_2(x_{s-1}) > r = \ranking_2(y_r) = \ranking_2(x_s)$. Thus, the relative rank of $x_{s-1}$ and $x_s$ under $\ranking_1$ and $\ranking_2$ differs. As $\ranking_1$ and $\ranking_2$ have the same execution trace, this means that the algorithm does not compare $x_{s-1}$ and $x_s$ on either input, and on $\ranking_1$ in particular. Let $\ranking'_1$ be the ranking obtained from ranking $\ranking_1$ by applying the adjacent-rank transposition $\transposition = (s-1,s)$. Since the algorithm does not compare the affected items, the execution trace for $\ranking'_1$ and $\ranking_1$ are the same, so $\ranking'_1 \in R$. We use $\transposition$ as our first step on the path from $\ranking_1$ to $\ranking_2$. What remains is to find a path from $\ranking'_1$ to $\ranking_2$. The situation is the same as the one depicted above but with $r$ increased by one in case $s=r+1$, and with the same $r$ and $s$ decreased by one, otherwise. The proof then follows by induction on the ordered pair $(r,n-s)$. 
\end{proof}

We already explained in Section~\ref{sec:overview} how the Connectivity Lemma shows that counting inversions and inversion parity amount to sorting, and require at least $\log(n!)$ queries. We now illustrate its use for a classical problem that is easier than sorting, namely median finding.

Let $\Pi$ denote the selection problem with rank $r = \ceil{n/2}$. For any ranking, the adjacent-rank transpositions $\transposition$ that change the item with rank $r$, are the two that involve rank $r$: $\transposition = (r-1,r)$ and $\transposition = (r,r+1)$. Those transpositions are the ones that correspond to missing edges in the permutahedron graph $G(\Pi)$. As a result, for any two rankings, there exists a path between them in $G(\Pi)$ if and only if they have the same median as well as the same set of items with rank less than $r$ (an d hence also the same set of items with rank greater than $r$). As there are $n$ possibilities for the median, and, for each median, $\binom{n-1}{r-1}$ possibilities for the set of items that have rank less than $r$, $G(\Pi)$ has $n \cdot \binom{n-1}{r-1}$ connected components. It follows that any algorithm for $\Pi$ has at least $n \cdot \binom{n-1}{r-1} = \Omega(\sqrt{n}\cdot 2^n)$ distinct execution paths, and therefore needs to make at least $n + \frac{1}{2} \log(n) - O(1)$ queries. 

As a side note, this example clarifies a subtlety in the equivalence between ordinary selection and the instantiation of partial order production that is considered equivalent to selection. Whereas selection of rank $r$ ordinarily requires outputting only the item
of rank $r$, the instantiation of partial order production additionally requires partitioning the remaining items according to whether their ranks are less than or greater than $r$. The above analysis implies that it is impossible for the algorithm to know the item of rank $r$ without also knowing how to partition the remaining items into those of rank less than and greater than $r$. It follows that, in the comparison-based model, ordinary selection and the instantiation of partial order production are equivalent. 


==> generalization.tex <==
\section{Generalization}
\label{sec:generalization}

In this section, we will analyze the sensitivity of trees with general shapes. Although the analysis in this section gives a weaker result than our bound in \cref{sec:binary} in the case of binary trees, it is applicable to far more general tree shapes. In particular, we can achieve the following bound on $k$-ary trees, where each node has at most $k$ children.

\begin{theorem}
    \label{thm:k-ary:sensitivity}
    Inversion minimization on a $k$-ary tree $T$ requires at least $\Omega(\frac{n}{k}\log(\frac{n}{k}))$ queries.
\end{theorem}

\subsection{Subtree Sensitivity}

We first introduce a sensitivity bound for inversion minimization based on the size of a subtree. 

\begin{lemma}[Subtree Sensitivity]
    \label{lemma:k-ary:subtree-sensitivity}
    Consider a tree $T$ with $n \doteq |L(T)|$ leaves, and some node $v\in T$ with $\ell \doteq |L(T_v)|$ leaves. We have
    \[s(\Pi_T) \ge \frac{\ell(n-\ell)}{n}-1. \]
\end{lemma}

Here, $v$ is not necessarily a direct child of the root, as shown in \cref{fig:k-ary:subtree}.

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \node (top) at (0,0)[circle, fill, inner sep=2pt, label={right:$r$}]{};
        \node (v) at (-0.5,-1.5)[circle, fill, inner sep=2pt, label={right:$v$}]{};
        \draw[decorate, decoration=snake, segment amplitude=1pt, segment length=2mm] (top)--(v);
        \draw[densely dotted, thick] (-2.1,-3.1) -- (top) -- (2.1,-3.1);
        \draw[densely dotted, thick] (-1.5,-3) -- (v) -- (0.5,-3);
        \draw (-2.1,-3.1)--(2.1,-3.1);
        \draw (-1.5,-3)--(0.5,-3);
        \node at (-0.5,-3.1)[label={$L(T_v)$}]{};
        \node at (0,-3)[label={below:$L(T)$}]{};
    \end{tikzpicture}
    \caption{Subtree rooted at $v$}
    \label{fig:k-ary:subtree}
\end{figure}

We now prove \cref{lemma:k-ary:subtree-sensitivity}. Let $\ranking$ be a ranking of the leaves of $T$, and let $\ordering_{\min}$ be a tree ordering that minimizes the number of inversions with respect to $\ranking$.

(WRITER'S NOTE) We are using the convention that $\ranking$ sends the ranking to the leaf.

\begin{claim}
    \label{claim:k-ary:decreasing-transposition}
    $\ranking$ is sensitive to the transposition $\transposition=(r,r+1)$ if $\ordering^{-1}_{\min}(\ranking(r))>\ordering^{-1}_{\min}(\ranking(r+1))$.
\end{claim}

\begin{proof}
    If $\ordering^{-1}_{\min}(\ranking(r))>\ordering^{-1}_{\min}(\rho(r+1))$, then $\Inv_{\transposition\circ\ranking}(\ordering_{\min})=\Inv_{\ranking}(\ordering_{\min})-1$. Since $\Inv_{\ranking}(\ordering_{\min})=\MInv(T,\ranking)$, this means that $\MInv(T,\transposition\circ\ranking)< \MInv(T,\ranking)$, or that $\ranking$ is sensitive to $\transposition$.
\end{proof}

In the case of general trees, a tree ordering $\ordering$ that minimizes the number of inversions with respect to $\ranking$ is difficult to find (see the discussion on NP-hardness in \cref{sec:turing}). Our strategy is to find a lower bound on the number of $r$ for which $\ordering^{-1}(\ranking(r))>\ordering^{-1}(\ranking(r+1))$ that applies regardless of $\ordering$.

\begin{proposition}
    \label{prop:k-ary:transposition-to-gap}
    For any ordering $\ordering$, the number of $r$ such that $\ordering^{-1}(\ranking(r))>\ordering^{-1}(\ranking(r+1))$ is at least one less than the number of $s$ such that $\ranking(s)\in L(T_v)$ and $\ranking(s+1)\not\in L(T_v)$.
\end{proposition}

\begin{proof}
    For all except at most one value of $s$ (the maximum $s$ for which $\ranking(s)\in L(T_v)$), there exists a minimal $s'>s$ such that $\ranking(s')\in L(T_v)$. We claim that at least one value of $r=s,\dots,s'-1$ satisfies $\sigma^{-1}(\ranking(r))>\sigma^{-1}(\ranking(r+1))$. If not, then $\ordering$ would rank $\ranking(s),\ranking(s+1),\dots,\ranking(s')$ in increasing order. Because $\ordering$ is a tree ordering, the leaves of $L(T_v)$ must be mapped into a contiguous range by $\ordering$, as shown in \cref{fig:k-ary:transposition-to-gap-visualization}. However, we have $\ranking(s),\ranking(s')\in L(T_v)$ but $\ranking(s+1)\not\in L(T_v)$, which violates this property since $\ordering$ ranks a leaf outside $L(T_v)$ between two leaves inside $L(T_v)$.
    
    Because each value of $r$ is found between consecutive pairs of values in $L(T_v)$, the values of $r$ are distinct.
\end{proof}

\begin{figure}
    \centering
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}
            [
            level 1/.style = {sibling distance = 4cm, level distance = 0.75cm},
            level 2/.style = {sibling distance = 1.5cm, level distance = 1cm},
            level 3/.style = {sibling distance = 1.4cm, level distance = 1cm},
            level 4/.style = {sibling distance = 0.9cm, level distance = 1cm}
            ]
            \node at (0,0)[circle, draw, inner sep=1.5pt]{}
                child
                {node [circle, draw, inner sep=1.5pt]{}
                    child
                    {node [circle, draw, inner sep=1.5pt, label={below:$2$}]{}}
                    child
                    {node [circle, draw, inner sep=1.5pt, label={below:$7$}]{}}}
                child
                {node [circle, draw, inner sep=1.5pt]{}
                    child
                    {node [circle, draw, inner sep=1.5pt, label={above:$v$}, sibling distance=3cm]{}
                        child
                        {node [circle, draw, inner sep=1.5pt]{}
                            child
                            {node [circle, fill, inner sep=1.5pt, label={below:$1$}]{}}
                            child
                            {node [circle, fill, inner sep=1.5pt, label={below:$5$}]{}}}
                        child
                        {node [circle, draw, inner sep=1.5pt]{}
                            child
                            {node [circle, fill, inner sep=1.5pt, label={below:$4$}]{}}
                            child
                            {node [circle, fill, inner sep=1.5pt, label={below:$6$}]{}}}
                        child
                        {node [circle, fill, inner sep=1.5pt, label={below:$8$}]{}}}
                    child
                    {node [circle, draw, inner sep=1.5pt, label={below:$3$}]{}}
                    child
                    {node [circle, draw, inner sep=1.5pt, label={below:$9$}]{}}};
        \end{tikzpicture}
        \caption{Leaves are arranged in $\ordering$-order, labeled with $\ranking$ values.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.45\textwidth}
        \centering
        \begin{tikzpicture}[scale=0.5, yscale=0.8]
            \draw[very thin, gray] (0,0) grid (10,10);
            \draw[->,thick] (0,0)--(10,0) node [label={below:$\ranking$}]{};
            \draw[->,thick] (0,0)--(0,10) node [label={left:$\ordering$}]{};
            \draw[dashed,thick] (0,3)--(10,3);
            \draw[dashed,thick] (0,7)--(10,7);
            \node at (0,5)[label={left:$L(T_v)$}]{};
            \draw[decorate, decoration=brace] (-0.3,3)--(-0.3,7);
            
            \node at (2.55,8.45){\scriptsize $r_1$};
            \node at (5.55,6.45){\scriptsize $r_2$};
            
            \node at (1,3)[circle, fill, inner sep=1.5pt]{};
            \node at (2,1)[circle, draw, fill=white, inner sep=1.5pt]{};
            \node at (3,8)[circle, draw, fill=white, inner sep=1.5pt]{};
            \node at (4,5)[circle, fill, inner sep=1.5pt]{};
            \node at (5,4)[circle, fill, inner sep=1.5pt]{};
            \node at (6,6)[circle, fill, inner sep=1.5pt]{};
            \node at (7,2)[circle, draw, fill=white, inner sep=1.5pt]{};
            \node at (8,7)[circle, fill, inner sep=1.5pt]{};
            \node at (9,9)[circle, draw, fill=white, inner sep=1.5pt]{};
            
            \draw (1.5,-0.76)--(3.5,-0.76);
            \draw (6.5,-0.76)--(7.5,-0.76);
            \node at (1,-0.76)[]{$s_1$};
            \node at (4,-0.67)[]{$s'_1$};
            \node at (6,-0.76)[]{$s_2$};
            \node at (8,-0.67)[]{$s'_2$};
        \end{tikzpicture}
        \caption{Corresponding plot of $\ranking,\ordering$ for each leaf.}
    \end{subfigure}
    \caption{$\ordering$ maps leaves of $L(T_v)$ in a contiguous range.}
    \label{fig:k-ary:transposition-to-gap-visualization}
\end{figure}

\begin{claim}
    \label{claim:k-ary:gap-count}
    Over a uniformly random $\ranking$, the expected number of $s$ such that $\ranking(s)\in L(T_v)$ and $\ranking(s+1)\not\in L(T_v)$ is $\frac{\ell(n-\ell)}{n}$.
\end{claim}

\begin{proof}
    For $s=1,\dots,n-1$, the probability that $\ranking(s)\in L(T_v)$ is $\frac{\ell}{n}$, and the probability that $\rho(s+1)\not\in L(T_v)$ given that $\ranking(s)\in L(T_v)$ is $\frac{n-\ell}{n-1}$. Using linearity of expectation on the indicator random variables for $\ranking(s)\in L(T_v)$ and $\ranking(s+1)\not\in L(T_v)$, the expected number of $s$ satisfying this property is
    \[(n-1)\left(\frac{\ell(n-\ell)}{n(n-1)}\right)=\frac{\ell(n-\ell)}{n}. \]
\end{proof}

Combining \cref{claim:k-ary:decreasing-transposition}, \cref{prop:k-ary:transposition-to-gap}, and \cref{claim:k-ary:gap-count}, we can conclude with \cref{lemma:k-ary:subtree-sensitivity}.

\subsection{$k$-ary Trees}

We can apply our analysis in the previous subsection to the case of $k$-ary trees. Observe that for fixed $n$, \cref{lemma:k-ary:subtree-sensitivity} is strongest when $\ell=n/2$. Not every tree $T$ will have a subtree with exactly $n/2$ leaves, but \cref{lemma:k-ary:subtree-sensitivity} still gives a useful bound for subtrees that do not contain too few or too many leaves. In the case of $k$-ary trees, there always exists a subtree $T_v$ that contains a reasonable amount of leaves.
 
\begin{fact}
    \label{fact:k-ary:balance}
    If $T$ is a $k$-ary tree, there exists a node $v\in T$ such that $\ell=cn$, where $\frac{1}{k+1} \le  c \le \frac{k}{k+1}$.
\end{fact}

\begin{proof}
    Let $r$ be the root of $T$, and construct a sequence $v_1=r,v_2,v_3,\dots$ such that $v_{i}$ is the child of $v_{i-1}$ that maximizes $\ell_{i}=|L(T_{v_{i}})|$, with ties broken arbitrarily. Notice that $\{\ell_i\}$ is a decreasing sequence, and since $T$ is a $k$-ary tree, $\ell_{i} \le k\ell_{i+1}$ for all $i$. We claim that some $v_i$ in this sequence satisfies the conditions of the claim. If not, then for some $i$, $\ell_i> \frac{k}{k+1}\cdot n$ and $\ell_{i+1}< \frac{1}{k+1}\cdot n$, which contradicts the fact that $\ell_i\le k\ell_{i+1}$.
\end{proof}

By choosing a subtree satisfying \cref{fact:k-ary:balance}, we can apply \cref{lemma:k-ary:subtree-sensitivity} to prove the following sensitivity bound on $k$-ary trees.

\begin{lemma}[$k$-ary Tree Sensitivity]
    \label{lemma:k-ary:sensitivity}
    For a $k$-ary tree $T$ with $n$ leaves,
    \[s(\Pi_T)\ge \frac{nk}{(k+1)^2}-1. \]
\end{lemma}

The Sensitivity Lemma (\cref{lemma:sensitivity}) gives \cref{thm:k-ary:sensitivity} as a result.



\subsection{Even leaf sets?}

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \node (top) at (0,0)[circle,draw,fill=black,inner sep=1.5pt,label={above:$v$}]{};
        \node (u1) at (-4,-1)[circle,draw,fill=black,inner sep=1.5pt]{};
        \node at (-2.75,-1){$\cdots$};
        \node (ulo) at (-1.5,-1)[circle,draw,fill=black,inner sep=1.5pt,label={left:$u_{\lo}$}]{};
        \node at (-0.75,-1){$\cdots$};
        \node (u2) at (0,-1)[circle,draw,fill=black,inner sep=1.5pt]{};
        \node at (0.75,-1){$\cdots$};
        \node (uhi) at (1.5,-1)[circle,draw,fill=black,inner sep=1.5pt,label={right:$u_{\hi}$}]{};
        \node at (2.75,-1){$\cdots$};
        \node (u3) at (4,-1)[circle,draw,fill=black,inner sep=1.5pt]{};
        
        
        \node (l1) at (-4,-3){};
        \node (llo) at (-1.5,-3)[circle,draw,fill=black,inner sep=1.5pt,label={below:$\ell_{\lo}$}]{};
        \draw[decorate, decoration=snake, segment amplitude=1pt, segment length=2mm] (ulo)--(llo);
        \node (l2) at (0,-3){};
        \node (lhi) at (1.5,-3)[circle,draw,fill=black,inner sep=1.5pt,label={below:$\ell_{\hi}$}]{};
        \draw[decorate, decoration=snake, segment amplitude=1pt, segment length=2mm] (uhi)--(lhi);
        \node (l3) at (4,-3){};
        
        \def\gap{0.6}
        \def\drop{2}
        \draw[densely dotted] (u1) ++({-\gap},{-\drop}) -- +({\gap},{\drop}) -- +({2*\gap},0);
        \draw (l1) ++({-\gap},0) -- +({2*\gap},0);
        \draw[densely dotted] (ulo) ++({-\gap},{-\drop}) -- +({\gap},{\drop}) -- +({2*\gap},0);
        \draw (llo) ++({-\gap},0) -- +({2*\gap},0);
        \draw[densely dotted] (u2) ++({-\gap},{-\drop}) -- +({\gap},{\drop}) -- +({2*\gap},0);
        \draw (l2) ++({-\gap},0) -- +({2*\gap},0);
        \draw[densely dotted] (uhi) ++({-\gap},{-\drop}) -- +({\gap},{\drop}) -- +({2*\gap},0);
        \draw (lhi) ++({-\gap},0) -- +({2*\gap},0);
        \draw[densely dotted] (u3) ++({-\gap},{-\drop}) -- +({\gap},{\drop}) -- +({2*\gap},0);
        \draw (l3) ++({-\gap},0) -- +({2*\gap},0);
        
        \draw (top)--(u1);
        \draw (top)--(ulo);
        \draw (top)--(u2);
        \draw (top)--(uhi);
        \draw (top)--(u3);
        
        \draw (-1,-0.05) .. controls (0,-0.4) .. (1,-0.05);
        \node at (0.8, -0.05)[label={right:$k$}]{};
    \end{tikzpicture}
    \caption{Sensitivity for General Trees}
    \label{fig:sensitivity-general}
\end{figure}

\paragraph{Higher degrees}

Consider an tree $T$ and a ranking $\ranking$ of its leaves. We have that
\begin{equation}\label{eq:MInv:sum}
\MInv(T,\ranking) = \sum_v \MRInv(T_v,\ranking), 
\end{equation}
where $v$ ranges over all internal nodes of $T$, and $\MRInv(T,\ranking)$ denotes the minimum number of inversions with respect to the ranking $\ranking$ that go through the \emph{root} of $T$, i.e., for which the affected leaves $\ell_1$ and $\ell_2$ have the root of $T$ as their lowest common ancestor. We have
\begin{equation}\label{eq:min:cost}
\MRInv(T,\ranking) = \min_\ordering \RInv(T,\ranking,\ordering), 
\end{equation}
where $\ordering$ ranges over the rankings of the children of $v$, and for a node $v$ with $k$ children $u_1,\dots,u_k$  and leaf sets $L_i \doteq L(T_{u_i})$ 
\begin{equation}\label{eq:cost}
\RInv(T,\ranking,\ordering) \doteq \sum_{1 \le i < j \le k} \XInv_\ranking(L_{\ordering(i)},L_{\ordering(j)}). 
\end{equation}

For a given ranking $\ranking$ of $T$ and a given adjacent-rank transposition $\transposition$, we would like to figure out the effect of $\tau$ on the objective $\MInv(T,\cdot)$, in particular when $\MInv(T,\transposition \circ \ranking) \ne \MInv(T,\ranking)$. The only term on the right-hand side of \eqref{eq:MInv:sum} that can be affected by the transposition $\transposition$ is the one corresponding to the node $v$ that is the least common ancestor $\LCA(\ell_1,\ell_2)$ of the two leaves $\ell_1$ and $\ell_2$ that are affected by $\transposition$ under $\ranking$. If $\ell_1$ and $\ell_2$ are children of $v$ itself, they can be freely swapped under $v$ and  $\RInv(T_v,\transposition \circ \ranking,\ordering) = \RInv(T_v,\ranking,\ordering)$ for any ordering $\ordering$, so $\transposition$ has no effect on $\MRInv(T_v,\cdot)$ nor on $\MInv(T,\cdot)$. Otherwise, $\ell_1$ and $\ell_2$ belong to the subtrees of distinct children of $v$. In this case, the transposition $\transposition$ changes the cost for any fixed $\ordering$ by one unit (up or down):
$|\RInv(T_v,\transposition \circ \ranking,\ordering) - \RInv(T_v,\ranking,\ordering)|=1$. It may still be the case that the minimum \eqref{eq:min:cost} remains unaffected, namely when the cost of an ordering $\ordering_1$ that is optimal for $\ranking$ goes up by one after transposition, and another ordering $\ordering_2$ that costs one unit more than $\ordering_1$ under $\ranking$ becomes one unit cheaper after transposition. To analyze the situation, let $\ell_\lo$ denote the smaller of the two affected leaves with respect to $\ranking$, and $\ell_\hi$ the other one, so we have $\ranking(\ell_\lo) < \ranking(\ell_\hi)$. Let $L_{i^*}$ be the set of leaves of a child of $v$ containing $\ell_\lo$, and similarly $L_{j^*}$ the leaf set containing $\ell_\hi$. In the situation under consideration, it has to be the case that $\ordering_1(i^*) < \ordering_1(j^*)$, $\ordering_2(i^*) > \ordering_2(j^*)$, and that 
\begin{equation}\label{eq:RInv:difference}
\RInv_\ranking(T_v,\ranking,\ordering_1) -
\RInv_\ranking(T_v,\ranking,\ordering_2) = -1 = \DInv_\ranking(\ell_\lo,\ell_\hi).
\end{equation}

We introduce some notation to facilitate the derivation.
For any two distinct leaves $x$ and $y$ of the underlying tree $T$
\[ \DInv_\ranking(\ell_1,\ell_2) \doteq \left\{ 
\begin{array}{ll} 
+1 & \rho(x) > \rho(y) \\
-1 & \rho(x) < \rho(y) 
% 0 & \textrm{otherwise}
\end{array} \right.
\]
and for disjoint sets $A$ and $B$ of leaves
\[ \DInv_\ranking(A,B) \doteq \sum\limits_{\substack{x \in A \\ y \in B}} \DInv_\rho(x,y).
\]
Note that $\DInv_\ranking(A,B) = \XInv_\ranking(A,B) - \XInv_\ranking(A,B)$, i.e., $\DInv_\ranking(A,B)$ equals the \emph{difference} of the cross inversions of $A$ to $B$ and the cross inversions the other way around. Since $\XInv_\ranking(A,B) + \XInv_\ranking(B,A) = |A| \cdot |B|$, we can express $\XInv_\ranking(A,B)$ in terms of  $\DInv_\ranking(A,B)$ as 
\begin{equation}\label{eq:XInv:DInv}
\XInv_\ranking(A,B) =  \frac{1}{2} \DInv_\ranking(A,B) + \frac{1}{2} |A| \cdot |B|.
\end{equation}
Using the above notation we can write
\begin{align}
\RInv_\ranking(T_v,\ranking,\ordering) 
& = \sum_{1 \le i < j \le k} \XInv_\ranking(L_i,L_j) \cdot \Indicator{\ordering(i) < \ordering(j)} \\
& \;\;\;\;\; + \sum_{1 \le i < j \le k} \XInv_\ranking(L_j,L_i) \cdot \Indicator{\ordering(i) > \ordering(j)} \\
& = \frac{1}{2} \sum_{1 \le i < j \le k} \left( \DInv_\ranking(L_i,L_j) \cdot (-1)^{\Indicator{\sigma(i > \sigma(j)}} + |L_1| \cdot |L_2| \right) \\
\RInv_\ranking(T_v,\ranking,\ordering_1) -
\RInv_\ranking(T_v,\ranking,\ordering_2)
& = 
\sum\limits_{\substack{1 \le i < j \le k \\ \ordering_1(i) < \ordering_2(j) \\ \ordering_2(i) > \ordering_2(j)}}\DInv_\ranking(L_i,L_j)
+ \sum\limits_{\substack{1 \le i < j \le k \\ \ordering_1(i) > \ordering_2(j) \\ \ordering_2(i) < \ordering_2(j)}} \DInv_\ranking(L_i,L_j)
\end{align}
By combination the last equation with \eqref{eq:RInv:difference} and separating out the term for $(i,j)=(i^*,j^*)$, we obtain the following criterion:
\begin{proposition}
Let $T$ be a tree, $\ranking$ a ranking of the leaves of $T$, $\transposition$ an adjacent-rank transposition, $\ell_\lo$ and $\ell_\hi$ the two leaves affected by $\transposition$ under $\ranking$ with $\ranking(\ell_\lo) < \ranking(\ell_\hi)$, $L_i, \dots, L_k$ the leaf sets of the children of $v = \LCA(\ell_\lo,\ell_\hi)$, $\ell_\lo \in L_{i^*}$, $\ell_\hi \in L_{j^*}$, and $\ordering_1$ and $\ordering_2$ two rankings of the children of $v$. Assuming that $v$ is not the parent of at least one of $\ell_\lo$ or $\ell_\hi$, and that $\ordering_1(i^*) < \ordering_1(j^*)$, the orderings $\ordering_1$ and $\ordering_2$ swap values for $\RInv(T_v,\ranking,\cdot)$ when $\transposition$ is applied to $\ranking$ iff
\begin{equation}\label{eq:necessary}
\DInv_\ranking(L_{i^*},L_{j^*}) - \DInv_\ranking(\ell_\lo,\ell_\hi)
= -\sum\limits_{\substack{1 \le i < j \le k \\ \ordering_1(i) < \ordering_2(j) \\ \ordering_2(i) > \ordering_2(j) \\ (i,j) \ne (i^*,j^*)}} \DInv_\ranking(L_i,L_j)
+ \sum\limits_{\substack{1 \le i < j \le k \\ \ordering_1(i) > \ordering_2(j) \\ \ordering_2(i) < \ordering_2(j)}} \DInv_\ranking(L_i,L_j).
\end{equation} 
\end{proposition}

By \eqref{eq:XInv:DInv}, the quantity $\DInv(L_i,L_j) + |L_i| \cdot |L_j|$ always is an even integer. If every leaf set is of size $|L_i|=k$ for $k$ even, this implies that $\DInv_\ranking(L_i,L_j)$ is even for all $1 \le i < j \le k$. As $\DInv_\ranking(\ell_\lo,\ell_\hi)$, it follows that the left-hand side of \eqref{eq:necessary} is odd, whereas the right-hand side is even -- a contradiction. We conclude that for perfect $k$-ary trees $T$ with $k$ even, the only adjacent-rank transpositions $\transposition$ that leave the objective $\MInv(T,\ranking)$ unchanged are those that swap leaves $\ell_\lo$ and $\ell_\hi$ that are siblings. 

Note: For the above argument we only need that all leave sets have even size, which happens iff all leaves have an odd number of siblings. 

The above sensitivity property does not hold for (all) odd values of $k$. Here is a counter-example with $k=3$. Consider the following ranking $\ranking$ of the leaves: (1,3,6,2,4,5,7,8,9). The minimum number of inversions equals 4. Consider the transposition $\tau$ that swaps ranks 3 and 4, resulting in the ranking (1,4,6,2,3,5,6,7,9). The minimum number of inversions remains at 4.

\paragraph{Replacing leaves by freely rearrangeable subtrees}


==> limitations.tex <==
\section{Limitations}
\label{sec:limitations}


==> sensitivity.tex <==
\section{Sensitivity Lemma}
\label{sec:sensitivity}

In this section we develop Lemma~\ref{lemma:sensitivity}.
We actually prove a somewhat stronger version.

\begin{lemma}[Strong Sensitivity Lemma]\label{lemma:sensitivity:strong}
Consider an algorithm $A$ in the comparison-based
model with $n$ items, color each vertex of the permutahedron with its execution trace under $A$, and let $\overline{H}$ denote the subgraph with the same vertex set but only containing the bichromatic edges. The number of distinct execution traces of $A$ is at least $g(\avgdeg(\overline{H})+1)/n$, where
% $\avgdeg(\overline{H})$ denotes the average degree of $\overline{H}$, and 
$g: [1,\infty) \to \mathbb{R}$ is any convex function with $g(x) = x!$ for $x \in [n]$.
\end{lemma}
The Sensitivity Lemma follows from Lemma~\ref{lemma:sensitivity:strong} because the coloring with execution traces of an algorithm $A$ for $\Pi$ is a refinement of the coloring with $\Pi$, so every edge of the permutahedron that is bichromatic under $\Pi$ is also bichromatic under $A$, and
\[
s(\Pi) \doteq \Expect[\deg_{\overline{G}(\Pi)}(\ranking)] \le \Expect[\deg_{\overline{H}}(\ranking)] \doteq \avgdeg(\overline{H}). 
\]
Provided $g$ is nondecreasing, it follows that $D(\Pi) \ge g(\avgdeg(\overline{H})+1)/n \ge g(s(\Pi)+1)/n$.

In the Sensitivity Lemma we set $g(x) = \Gamma(x+1)$. An optimal (but less elegant) choice for $g$ is the piece-wise linear function that interpolates the prescribed values at the integral points in $[n]$, namely
\[    g(x) \doteq
      (x - \floor{x})\cdot(\ceil{x}!)
      +
      (1 - (x - \floor{x}))\cdot(\floor{x}!).
\]      

For the proof of Lemma~\ref{lemma:sensitivity:strong} we take intuition from a similar result in the Boolean setting \cite[Exercise~8.43]{ODonnell2014}.
\begin{fact}\label{fact:Boolean} 
Let $A$ be a query algorithm on binary strings of length $n$. Color each vertex of the $n$-dimensional hypercube by its execution trace under $A$, and let $\overline{H}$ denote the subgraph with the same vertex set but only containing the bichromatic edges. Then the number of distinct execution traces is at least $2^{\avgdeg(H)}$.
\end{fact}

One way to argue Fact~\ref{fact:Boolean} is to think of assigning a weight $w(x)$ to each $x \in \{0,1\}^n$ so as to maximize the total weight on all inputs, subject to the constraint that the total weight on each individual execution trace is at most 1. Then the number of distinct execution traces must be at least the sum of all the weights. If the weight only depends on the degree, i.e., if we can write $w(x) = f(\deg_{\overline{H}}(x)$ for some function $f: [0,\infty) \to \mathbb{R}$, then we can lower bound the number $k$ of distinct execution traces as follows:
\begin{equation}\label{eq:Boolean}
k \ge \sum_x w(x) = \sum_x f(\deg_{\overline{H}}(x)) \ge 2^n \cdot f(\Expect[\deg(x)]) = 2^n \cdot f(\avgdeg(\overline{H})),
\end{equation}
where the last step holds provided $f$ is convex. 

In the Boolean setting the set $R$ of inputs $x \in \{0,1\}^n$ with a particular execution trace forms a subcube of dimension $n-\ell$, where $\ell$ denotes the length of the execution trace, i.e., the number of queries. Each $x \in R$ has degree $\ell$ in $H$; this is because a change in a single queried position results in a different execution trace, and a change in another position does not. Therefore, a natural choice for the weight of $x \in R$ is $w(x) = f(\ell)$ where $f(x) = 1/2^{n-\ell}$. It satisfies the constraint that the total weight on $R$ is (at most) one, and $f$ is convex. We conclude by \eqref{eq:Boolean} that the number of distinct execution traces is at least $2^n \cdot f(\avgdeg(\overline{H})) = 2^{\avgdeg(\overline{H})}$, as desired.

\begin{proof}[Proof of Lemma~\ref{lemma:sensitivity:strong}]
Let $k$ denote the number of distinct execution traces of $A$, and let $R_1, \dots, R_k$ denote the corresponding sets of rankings. 
Following a similar strategy, we want to find a convex function $f: [0,\infty)$ such that the weight function $w(\ranking) = f(\deg_{\overline{H}}(\ranking))$ does not assign weight more than 1 to any particular of the sets $R_i$. The following claim, to be proven later, is the crux of this.

\begin{claim}\label{claim:encoding}
Let $R$ denote the set of all rankings $\ranking$ that follow a particular execution trace on $A$, and let $d \in \{0,\dots,n-1\}$. The number of rankings $\ranking \in R$ with $\deg_{\overline{H}}(\ranking) = d$ is at most $\frac{n!}{(d+1)!}$.
\end{claim}

Based on Claim~\ref{claim:encoding}, a natural choice for $f$ is any convex function that satisfies $f(x) = \frac{1}{n} \frac{(x+1)!}{n!}$ for $x \in \{0,\dots,n-1\}$. For every $i \in [k]$ we then have
\[ \sum_{\ranking \in R_i} w(\ranking) = \sum_{d=0}^{n-1} \left| \{ \ranking \in R_i \, : \, \deg_{\overline{H}}(\ranking) = d \} \right| \cdot f(d) \le \sum_{d=0}^{n-1} \frac{1}{n} \frac{(x+1)!}{n!} \cdot \frac{n!}{(d+1)!} = \sum_{d=0}^{n-1} \frac{1}{n} = 1. \]
Similar to \eqref{eq:Boolean} we conclude
\begin{equation}\label{eq:lb:k}
k \ge \sum_{i=1}^k \sum_{\ranking \in R_i} w(\ranking) 
= \sum_\ranking w(\ranking)
= \sum_\ranking f(\deg_{\overline{H}}(\ranking)) \ge n! \cdot f(\Expect[\deg_{\overline{H}}(\ranking)]) = n! \cdot f(\avgdeg(\overline{H})). 
\end{equation}
Setting $f(x) = \frac{1}{n} \frac{g(x+1)}{n!}$ turns the requirements for $f$ into those for $g$ in the statement of the lemma, and yields that $k \ge n! \cdot f(\avgdeg(\overline{H})) = g(\avgdeg(\overline{H})+1)/n$. 
\end{proof}

We now turn to proving Claim~\ref{claim:encoding}. The comparisons and outcomes that constitute a particular execution trace of $A$ can be thought of as directed edges between the items in $X$. We refer to the resulting digraph on the vertex set $X$ as the comparison graph $C$. Since the outcomes of the comparisons are consistent with some underlying ranking, the digraph $C$ is acyclic. The rankings in $R$ are in one-to-one and onto correspondence with the linear orderings of the DAG $C$. For a given ranking $\ranking \ in R$, the degree $\deg_{\overline{H}}(\ranking)$ equals the number of $r \in \{2,\dots,n\}$ such that swapping ranks $r-1$ and $r$ in $\ranking$ results in a ranking $\ranking' = \ranking \circ \transposition$ that is not in $R$, where $\transposition$ denotes the adjacent-rank transposition $(r-1,r)$. The ranking $\ranking'$ not being in $R$ means that it is inconsistent with the combined comparisons and outcomes of the underlying execution trace, which happens exactly when there is a path in $C$ from the item $\ranking(r-1)$ of rank $r-1$ in $\ranking$ to the item $\ranking(r)$ with rank $r$ in $\ranking$. Thus, the degree $\deg_{\overline{H}}(\ranking)$ equals the number of $r \in \{2,\dots,n\}$ such that there is a path from $\ranking(r-1)$ to $\ranking(r)$ in $C$. See Figure~\ref{fig:encoding} for an illustration, where a squiggly edge $u \leadsto v$ denotes that there exists a path from $u$ to $v$ in $C$. We only draw squiggly edges from one position to the next, so $\deg_{\overline{H}}(\ranking)$ equals the number of squiggly edges in Figure~\ref{fig:encoding}. 

\begin{figure}[h]
    \centering
    \begin{tikzpicture}
        \node at (0,0)[]{rank};
        \node at (1,0)[]{$1$};
        \node at (2,0)[]{$2$};
        \node at (3,0)[]{$3$};
        \node at (4,0)[]{$4$};
        \node at (5,0)[]{$5$};
        \node at (6,0)[]{$\dots$};
        \node at (7,0)[]{$r-1$};
        \node at (8,0)[]{$r$};
        \node at (9,0)[]{$\dots$};
        \node at (10,0)[]{$n$};
        
        \node at (0,-0.8)[]{$\ranking$};
        \node (1) at (1,-0.8)[circle, fill, inner sep=1.5pt]{};
        \node (2) at (2,-0.8)[circle, draw, inner sep=1.5pt]{};
        \node (3) at (3,-0.8)[circle, fill, inner sep=1.5pt]{};
        \node (4) at (4,-0.8)[circle, fill, inner sep=1.5pt]{};
        \node (5) at (5,-0.8)[circle, draw, inner sep=1.5pt]{};
        \node (r) at (7,-0.8)[circle, draw, inner sep=1.5pt]{};
        \node (r1) at (8,-0.8)[circle, fill, inner sep=1.5pt]{};
        \node (n) at (10,-0.8)[circle, draw, inner sep=1.5pt]{};
        
        \draw[->, decorate, decoration=snake, segment amplitude=1pt, segment length=2.2mm] (2)--(3);
        \draw[->, decorate, decoration=snake, segment amplitude=1pt, segment length=2.2mm] (3)--(4);
        \draw[->, decorate, decoration=snake, segment amplitude=1pt, segment length=2.2mm] (r)--(r1);

    \end{tikzpicture}
\caption{Ranking encoding}\label{fig:encoding}
\end{figure}

Our strategy is to give a \emph{compressed encoding} of the rankings in $R$ such that there is more compression as the number of squiggly edges increases. Our encoding is based on the well-known algorithm to compute a linear order of a DAG. Algorithm~\ref{alg:linear-order} provides pseudocode for
the algorithm, which we refer to as BuildRanking.

\begin{algorithm}[ht]
  \caption{BuildRanking$(C)$}\label{alg:linear-order}
  \begin{algorithmic}[1]
    \Require DAG $C$ on vertex set $X$
    \Ensure ranking of $X$ that is a linear order of $C$
    \State $T \gets \varnothing$
%    \State $S \gets \{ v \in X \;\mid\; \text{there is no } u \in X \setminus T \text{ with } u \leadsto v \text{ in } G \}$
    \For{\(r=1\) to \(n\)}
      \State \label{alg:linear-order:step}%
      $x \gets$ arbitrary element of $S \doteq  \{ v \in X \;\mid\; \text{there is no } u \in X \setminus T \text{ with } u \leadsto v \text{ in } G \}$
      \State $\ranking(r) \gets x$ 
      \State $T \gets T \cup \{x\}$
    \EndFor
  \end{algorithmic}
\end{algorithm}

In our formulation, BuildRanking is nondeterministic: There is a choice to make in step~\ref{alg:linear-order:step} for each $r=1,\dots,n$. The possible executions of BuildRanking are in one-to-one and onto correspondence with the linear orders of $C$, and thus with the rankings in $R$. 

Our encoding is a compressed description of how to make the decisions in BuildRanking such that the output is $\ranking$. Note that if $\ranking(r-1) \leadsto \ranking(r)$, then item $x = \ranking(r)$ cannot enter the set $S$ before iteration $r$. This is because before $\ranking(r-1)$ is removed from $T$ at the end of iteration $r-1$, the edge $\ranking(r-1) \leadsto \ranking(r)$ prevents $x$ from being in $S$. Thus, whenever $\ranking(r-1) \leadsto \ranking(r)$, the item $x=\ranking(r)$ is \emph{lucky} in the sense that it gets picked in step~\ref{alg:linear-order:step} as soon as it enters the set $S$. In fact, the lucky items with respect to a ranking $\ranking \in R$ are exactly those for which $\ranking(r-1) \leadsto \ranking(r)$ for some $r \in \{2,\dots,n\}$, as well as the item $\ranking(1)$. In Figure~\ref{fig:encoding} the lucky items are marked black. Their number equals $\deg_{\overline{H}}(\ranking)+1$. 

In order to generate ranking $\ranking$ using BuildRanking, it suffices to know:
\begin{itemize}
\item[(a)] the lucky items (as a the set, not their relative ordering), and 
\item[(b)] the ordering of the non-lucky items (given which items they are).
\end{itemize}
This information suffices to make the correct choices in step~\ref{alg:linear-order:step} of Algorithm~\ref{alg:linear-order}:
\begin{itemize}
\item 
If the set $S$ contains a lucky item, there will be a unique lucky item in  $S$; pick it as the element $x$.
\item 
Otherwise, pick for $x$ the first item in the ordering of the non-luck items that is not yet in $T$. Such an element will exist, and all the items that come after it in the ordering are not yet in $T$ either.
\end{itemize}
If $\ranking$ has degree $d = \deg_{\overline{H}}(\ranking)$, there are $d+1$ luck items, so there are at most $\binom{n}{d+1}$ choices for (a), and at most $(n-d-1)!$ choices for (b), resulting in a total of at most $\binom{n}{d+1} \cdot (n-d-1)! = \frac{n!}{(d+1)!}$ choices. This proves Claim~\ref{claim:encoding}.

\begin{remark}\label{remark:sensitivity}
Suppose we allow an algorithm $A$ to have multiple valid execution traces on a given input $\ranking$, and let $R_i$ denote the set of rankings on which the $i$-th execution trace is valid. The proof of Claim~\ref{claim:encoding} carries over as it considers individually sets $R_i$, and only depends on the DAG that the comparisons in $R_i$ induce. The rest of the proof of Lemma~\ref{lemma:sensitivity:strong} carries through modulo the first equality in \eqref{eq:lb:k}, which no longer holds as the sets $R_i$ may overlap. However, the equality can be replaced by the inequality $\ge$, which does hold and is sufficient for the argument. This means that we can replace $D(\Pi)$ in the statement of the Sensitivity Lemma by its nondeterministic variant $N(\Pi)$.
\end{remark}

